Doubles melanges des polylogarithmes multiples aux racines de l'unit'e

The values at positive integers of the polyzeta functions are solutions of the polynomial equations arising from Drinfeld's associators, which have numerous applications in quantum algebra. Considered as iterated integrals they become periods of the motivic fundamental groupoid of $\mathbb{P}^1\setminus\{0,1,\infty\}$. From there comes a fundamental, yet no more explicit, system of algebraic relations; it implies the system of associators. We focus here on the combinatorics properties of another system of relations, the ``double shuffles'', which comes from elementary series and integrals manipulations. We show that it shares a torsor property with associators and ``motivic'' relations, is implied by the latter and defines a polynomial algebra over $\mathbb{Q}$ (a result first due to J. Ecalle). We obtain these results for more general numbers: values of Goncharov's multiple polylogarithms at roots of unity. These results were previously announced in math.QA:0012024. Here is the detailed proof.

==> carac.tex <==
\usepackage{mathrsfs}

\def \AM{{\mathbb{A}}}
\def \BM{{\mathbb{B}}}
\def \CM{{\mathbb{C}}}
\def \DM{{\mathbb{D}}}
\def \EM{{\mathbb{E}}}
\def \FM{{\mathbb{F}}}
\def \GM{{\mathbb{G}}}
\def \HM{{\mathbb{H}}}
\def \IM{{\mathbb{I}}}
\def \JM{{\mathbb{J}}}
\def \KM{{\mathbb{K}}}
\def \LM{{\mathbb{L}}}
\def \Mm{{\mathbb{M}}}
\def \NM{{\mathbb{N}}}
\def \OM{{\mathbb{O}}}
\def \PM{{\mathbb{P}}}
\def \QM{{\mathbb{Q}}}
\def \RM{{\mathbb{R}}}
\def \SM{{\mathbb{S}}}
\def \TM{{\mathbb{T}}}
\def \UM{{\mathbb{U}}}
\def \VM{{\mathbb{V}}}
\def \WM{{\mathbb{W}}}
\def \XM{{\mathbb{X}}}
\def \YM{{\mathbb{Y}}}
\def \ZM{{\mathbb{Z}}}

\def \AC{{\mathcal A}}
\def \BC{{\mathcal B}}
\def \CC{{\mathcal C}}
\def \DC{{\mathcal D}}
\def \EC{{\mathcal E}}
\def \FC{{\mathcal F}}
\def \GC{{\mathcal G}}
\def \HC{{\mathcal H}}
\def \IC{{\mathcal I}}
\def \JC{{\mathcal J}}
\def \KC{{\mathcal K}}
\def \LC{{\mathcal L}}
\def \MC{{\mathcal M}}
\def \NC{{\mathcal N}}
\def \OC{{\mathcal O}}
\def \PC{{\mathcal P}}
\def \QC{{\mathcal Q}}
\def \RC{{\mathcal R}}
\def \SC{{\mathcal S}}
\def \TC{{\mathcal T}}
\def \UC{{\mathcal U}}
\def \VC{{\mathcal V}}
\def \WC{{\mathcal W}}
\def \XC{{\mathcal X}}
\def \YC{{\mathcal Y}}
\def \ZC{{\mathcal Z}}

\def \AG{{\mathfrak A}}
\def \BG{{\mathfrak B}}
\def \CG{{\mathfrak C}}
\def \DG{{\mathfrak D}}
\def \EG{{\mathfrak E}}
\def \FG{{\mathfrak F}}
\def \GG{{\mathfrak G}}
\def \HG{{\mathfrak H}}
\def \IG{{\mathfrak I}}
\def \JG{{\mathfrak J}}
\def \KG{{\mathfrak K}}
\def \LG{{\mathfrak L}}
\def \MG{{\mathfrak M}}
\def \NG{{\mathfrak N}}
\def \OG{{\mathfrak O}}
\def \PG{{\mathfrak P}}
\def \QG{{\mathfrak Q}}
\def \RG{{\mathfrak R}}
\def \SG{{\mathfrak S}}
\def \TG{{\mathfrak T}}
\def \UG{{\mathfrak U}}
\def \VG{{\mathfrak V}}
\def \WG{{\mathfrak W}}
\def \XG{{\mathfrak X}}
\def \YG{{\mathfrak Y}}
\def \ZG{{\mathfrak Z}}

\def \aG{{\mathfrak a}}
\def \bG{{\mathfrak b}}
\def \cG{{\mathfrak c}}
\def \dG{{\mathfrak d}}
\def \eG{{\mathfrak e}}
\def \fG{{\mathfrak f}}
\def \gG{{\mathfrak g}}
\def \hG{{\mathfrak h}}
\def \iG{{\mathfrak i}}
\def \jG{{\mathfrak j}}
\def \kG{{\mathfrak k}}
\def \lG{{\mathfrak l}}
\def \mG{{\mathfrak m}}
\def \nG{{\mathfrak n}}
\def \oG{{\mathfrak o}}
\def \pG{{\mathfrak p}}
\def \qG{{\mathfrak q}}
\def \rG{{\mathfrak r}}
\def \sG{{\mathfrak s}}
\def \tG{{\mathfrak t}}
\def \uG{{\mathfrak u}}
\def \vG{{\mathfrak v}}
\def \wG{{\mathfrak w}}
\def \xG{{\mathfrak x}}
\def \yG{{\mathfrak y}}
\def \zG{{\mathfrak z}}

\def \ACC{{\mathscr A}}
\def \BCC{{\mathscr B}}
\def \CCC{{\mathscr C}}
\def \DCC{{\mathscr D}}
\def \ECC{{\mathscr E}}
\def \FCC{{\mathscr F}}
\def \GCC{{\mathscr G}}
\def \HCC{{\mathscr H}}
\def \ICC{{\mathscr I}}
\def \JCC{{\mathscr J}}
\def \KCC{{\mathscr K}}
\def \LCC{{\mathscr L}}
\def \MCC{{\mathscr M}}
\def \NCC{{\mathscr N}}
\def \OCC{{\mathscr O}}
\def \PCC{{\mathscr P}}
\def \QCC{{\mathscr Q}}
\def \RCC{{\mathscr R}}
\def \SCC{{\mathscr S}}
\def \TCC{{\mathscr T}}
\def \UCC{{\mathscr U}}
\def \VCC{{\mathscr V}}
\def \WCC{{\mathscr W}}
\def \XCC{{\mathscr X}}
\def \YCC{{\mathscr Y}}
\def \ZCC{{\mathscr Z}}


\def\aB{\mathbf{a}}
\def\bB{\mathbf{b}}
\def\cB{\mathbf{c}}
\def\dB{\mathbf{d}}
\def\eB{\mathbf{e}}
\def\fB{\mathbf{f}}
\def\gB{\mathbf{g}}
\def\hB{\mathbf{h}}
\def\iB{\mathbf{i}}
\def\jB{\mathbf{j}}
\def\kB{\mathbf{k}}
\def\lB{\mathbf{l}}
\def\mB{\mathbf{m}}
\def\nB{\mathbf{n}}
\def\oB{\mathbf{o}}
\def\pB{\mathbf{p}}
\def\qB{\mathbf{q}}
\def\rB{\mathbf{r}}
\def\sB{\mathbf{s}}
\def\tB{\mathbf{t}}
\def\uB{\mathbf{u}}
\def\vB{\mathbf{v}}
\def\wB{\mathbf{w}}
\def\xB{\mathbf{x}}
\def\yB{\mathbf{y}}
\def\zB{\mathbf{z}}
\def\AB{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CB{\mathbf{C}}
\def\DB{\mathbf{D}}
\def\EB{\mathbf{E}}
\def\FB{\mathbf{F}}
\def\GB{\mathbf{G}}
\def\HB{\mathbf{H}}
\def\IB{\mathbf{I}}
\def\JB{\mathbf{J}}
\def\KB{\mathbf{K}}
\def\LB{\mathbf{L}}
\def\MB{\mathbf{M}}
\def\NB{\mathbf{N}}
\def\OB{\mathbf{O}}
\def\PB{\mathbf{P}}
\def\QB{\mathbf{Q}}
\def\RB{\mathbf{R}}
\def\SB{\mathbf{S}}
\def\TB{\mathbf{T}}
\def\UB{\mathbf{U}}
\def\VB{\mathbf{V}}
\def\WB{\mathbf{W}}
\def\XB{\mathbf{X}}
\def\YB{\mathbf{Y}}
\def\ZB{\mathbf{Z}}

